LDTR: Transformer-based Lane Detection with Anchor-chain Representation

Despite recent advances in lane detection methods, scenarios with limited- or no-visual-clue of lanes due to factors such as lighting conditions and occlusion remain challenging and crucial for automated driving. Moreover, current lane representations require complex post-processing and struggle with specific instances. Inspired by the DETR architecture, we propose LDTR, a transformer-based model to address these issues. Lanes are modeled with a novel anchor-chain, regarding a lane as a whole from the beginning, which enables LDTR to handle special lanes inherently. To enhance lane instance perception, LDTR incorporates a novel multi-referenced deformable attention module to distribute attention around the object. Additionally, LDTR incorporates two line IoU algorithms to improve convergence efficiency and employs a Gaussian heatmap auxiliary branch to enhance model representation capability during training. To evaluate lane detection models, we rely on Frechet distance, parameterized F1-score, and additional synthetic metrics. Experimental results demonstrate that LDTR achieves state-of-the-art performance on well-known datasets.

==> latexmkrc <==
# vim: set ft=perl:

@default_files=('main', 'appendix');

$pdf_mode=1;
$pdflatex="pdflatex -interaction=nonstopmode -file-line-error -halt-on-error -synctex=1 %O %S";
$out_dir="./out";

$bibtex_use=1.5;

$clean_ext="thm bbl hd synctex.gz";

$makeindex="makeindex -s gind.ist %O -o %D %S";
add_cus_dep('glo', 'gls', 0, 'makeglo2gls');
sub makeglo2gls {
    system("makeindex -s gglo.ist -o \"$_[0].gls\" \"$_[0].glo\"");
}
push @generated_exts, "glo", "gls";

